Free-Grained Hierarchical Visual Recognition

Hierarchical image recognition seeks to predict class labels along a semantic taxonomy, from broad categories to specific ones, typically under the tidy assumption that every training image is fully annotated along its taxonomy path. Reality is messier: A distant bird may be labeled only bird, while a clear close-up may justify bald eagle. We introduce free-grain training, where labels may appear at any level of the taxonomy and models must learn consistent hierarchical predictions from incomplete, mixed-granularity supervision. We build benchmark datasets with varying label granularity and show that existing hierarchical methods deteriorate sharply in this setting. To make up for missing supervision, we propose two simple solutions: One adds broad text-based supervision that captures visual attributes, and the other treats missing labels at specific taxonomy levels as a semi-supervised learning problem. We also study free-grained inference, where the model chooses how deep to predict, returning a reliable coarse label when a fine-grained one is uncertain. Together, our task, datasets, and methods move hierarchical recognition closer to the way labels arise in the real world.

==> floats/suppl_fig_saliency_1.tex <==
\begin{figure*}[h]
%
\small\centering
\newcommand{\squareimage}[1]{\includegraphics[width=0.13\linewidth, height=0.13\linewidth]{#1}}
%
\newcommand{\colspace}{\hspace{5pt}}
\newcommand{\colspaceclose}{\hspace{3pt}}

\newcommand{\tablerow}[1]{
\squareimage{figures/attention_imgs/#1.jpg} &
\squareimage{figures/attention_imgs/#1_CHMatchModule_basic.jpg} &
\squareimage{figures/attention_imgs/#1_CHMatchModule_subordinate.jpg} &
\squareimage{figures/attention_imgs/#1_CHMatchModule_finegrained.jpg} &
\squareimage{figures/attention_imgs/#1_HierVisionTransformer_basic.jpg} &
\squareimage{figures/attention_imgs/#1_HierVisionTransformer_subordinate.jpg} &
\squareimage{figures/attention_imgs/#1_HierVisionTransformer_finegrained.jpg}

}
%
\resizebox{1.0\linewidth}{!}{
\begin{tabular}
{@{}
c@{\colspace}
c@{\colspaceclose}c@{\colspaceclose}c@{\colspace} |
c@{\colspaceclose}c@{\colspaceclose}c@{}
}
&
\multicolumn{3}{c}{\methodSSL} &
\multicolumn{3}{c}{Text-Attr} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
Image & 
\levelCoarse & \levelMid & \levelFG &
\levelCoarse & \levelMid & \levelFG \\%[-10pt]
%
\tablerow{162654}\\[-1pt]
% \levelFG &
&
bird \greencmark & \footnotesize{gallinaceous bird} \redxmark & junco \greencmark &
bird \greencmark & \footnotesize{passerine bird} \greencmark & junco \greencmark \\[1pt]

\tablerow{616936}\\[-1pt]
% \levelFG &
&
vehicle \greencmark & van \greencmark & police van \greencmark &
vehicle \greencmark & van \greencmark & police van \greencmark \\[1pt]
%
\tablerow{192972}\\[-1pt]
% \levelFG &
&
bird \greencmark & wading bird \greencmark & white stork \greencmark &
bird \greencmark & wading bird \greencmark & white stork \greencmark \\[1pt]

\tablerow{225554}\\[-1pt]
% \levelFG &
&
fish \greencmark & ganoid fish \greencmark & electric ray \redxmark &
fish \greencmark & ganoid fish \greencmark & gar \greencmark \\
% \tablerow{162500}\\[-1pt]
% % \levelFG &
% &
% bird \greencmark & \footnotesize{gallinaceous bird} \redxmark & junco \greencmark &
% bird \greencmark & \footnotesize{passerine bird} \greencmark & junco \greencmark \\[1pt]
%
%


%
% \tablerow{188499}\\[-1pt]
% % \levelFG &
% &
% bird \greencmark & wading bird \greencmark & \tiny{red-backed sandpiper} \greencmark &
% bird \greencmark & wading bird \greencmark & \tiny{red-backed sandpiper} \greencmark \\[1pt]

%
\tablerow{460831}\\[-1pt]
% \levelMid &
&
music instru. \greencmark & wind instru. \greencmark & flute \redxmark &
music instru. \greencmark & wind instru. \greencmark & harmonica \redxmark \\[1pt]



%

\tablerow{578213}\\[-1pt]
% \levelFG &
&
vehicle \greencmark & car \greencmark & convertible \greencmark &
vehicle \greencmark & car \greencmark & convertible \greencmark \\[1pt]
%
%
\tablerow{90235}\\[-1pt]
% \levelMid &
&
clothing \redxmark & bottoms \redxmark & kimono \redxmark &
dog \greencmark & terrier dog \greencmark & boston terrier \greencmark  \\[1pt]


% \tablerow{241402}\\[-1pt]
% % \levelFG &
% &
% fish \greencmark & \footnotesize{spiny-finned fish} \greencmark & lion fish \greencmark &
% fish \greencmark & \footnotesize{spiny-finned fish} \greencmark & lion fish \greencmark \\[1pt]
% %
% \tablerow{138810}\\[-1pt]
% % \levelFG &
% &
% bird \greencmark & \footnotesize{gallinaceous bird} \greencmark & black grouse \greencmark &
% bird \greencmark & \footnotesize{gallinaceous bird} \greencmark & black grouse \greencmark \\[1pt]


%


%
%
\end{tabular}
}
\caption{\textbf{Saliency map visualization of \methodSSL and Text-Attr.}}
\label{fig:suppl_saliency_1}
\vspace{-5pt}
\end{figure*}
